What makes a good metric? Evaluating automatic metrics for text-to-image consistency

Language models are increasingly being incorporated as components in larger AI systems for various purposes, from prompt optimization to automatic evaluation. In this work, we analyze the construct validity of four recent, commonly used methods for measuring text-to-image consistency - CLIPScore, TIFA, VPEval, and DSG - which rely on language models and/or VQA models as components. We define construct validity for text-image consistency metrics as a set of desiderata that text-image consistency metrics should have, and find that no tested metric satisfies all of them. We find that metrics lack sufficient sensitivity to language and visual properties. Next, we find that TIFA, VPEval and DSG contribute novel information above and beyond CLIPScore, but also that they correlate highly with each other. We also ablate different aspects of the text-image consistency metrics and find that not all model components are strictly necessary, also a symptom of insufficient sensitivity to visual information. Finally, we show that all three VQA-based metrics likely rely on familiar text shortcuts (such as yes-bias in QA) that call their aptitude as quantitative evaluations of model performance into question.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_experiments_section_mar27.tex <==
\section{Experiment 1: Relationship with linguistic properties}\label{sec:corr-ling}

An ideal \metric would draw on information from the prompt and from the image. To determine whether the \metrics are highly dependent on the prompt in particular, we evaluate the correlation between the \metrics and several standard linguistic properties of the text prompt or questions. We measure Spearman's rank correlation between the \metric and the \textbf{readability}, \textbf{complexity}, \textbf{length} of the prompt. For readability, we use the Flesch–Kincaid grade level calculation \citep{flesch1948new}. Flesch-Kincaid approximates the difficulty of reading a passage, based in part on word and sentence length, with higher scores corresponding to more difficulty. For complexity, we use Yngve scores \citep{yngve1960model}.  Yngve scores use constituency parsing, where deeper and wider of parse trees means more complex sentences. Finally, for prompt length, we use the number of words as tokenization using NLTK's word tokenizer \citep{loper2002nltk}. We exclude stopwords from the word count.

Results are shown in Table \ref{tab:linguistic-corr-coco} for COCO and in Table \ref{tab:ling-corr-winoground} for Winoground in the Appendix. Overall, we find that all metrics are correlated to a medium-to-strong degree with all linguistic properties for COCO and for length for Winoground, suggesting that the \metrics are sensitive to the properties of the text prompts. CLIPScore is not particularly sensitive to syntactic complexity but does positively correlate with grade-level and prompt length. On the contrary, the VQA-based metrics all \textit{negatively} correlate with the linguistic properties. % This fits our intuition, that the generally ``harder" prompts (longer, more complex, higher grade-level) score lower on the metrics.



\paragraph{Do \metrics correlate with prompt readability?} We approximate the readability of using prompt using the Flesch–Kincaid grade level calculation \citep{flesch1948new}. Flesch-Kincaid approximates the difficulty of reading a passage, based in part on word and sentence length, with higher scores corresponding to more difficulty. Results are shown in Table \ref{tab:linguistic-corr-coco}. We find a medium to strong negative correlation between grade level readability and metric scores for TIFA, VPEval, and DSG.

\paragraph{Do \metrics correlate with prompt syntactic complexity?} Syntactic complexity represents the difficulty of parsing a sentence, with higher difficulty correlating with lower scores. %We hypothesize that more syntactically difficult prompts would correlate with lower metric scores.
We use Yngve scores \citep{yngve1960model} to approximate the complexity of the syntactic complexity of prompts. Yngve scores use constituency parsing, where deeper and wider of parse trees means more complex sentences. Results are shown in Table \ref{tab:linguistic-corr-coco}.
We find a strong negative correlation between complexity and scores (more complex sentences mean lower scores) for all of the VQA based metrics. This lack of correlation is likely because CLIP is not strongly order-dependent and largely functions as a bag-of-words model \citep{yuksekgonul2022and}.


\paragraph{Do \metrics\ correlate with prompt length?} We measure sentence length as the number of words in the prompt using NLTK's word tokenizer \citep{loper2002nltk}. We observe a high negative correlation between length and the metric scores for TIFA, VPEval, and DSG. This effect presumably arises from the fact that longer captions generally have more content which needs to be generated, and therefore, the model might leave something out that is targeted by a question. Compare the existing COCO caption, ``A big burly grizzly bear is shown with grass in the background'' with another caption ``a big bear''. The latter is much less specific than the former: the bear could be grey, the bear could be skinny, the bear could be walking on ice, etc. In principle, the former, more specific caption has more constraints on what should be generated, and thus we might expect a lower score for the more difficult generation.

%\paragraph{Do evaluation metrics correlate with frequency of prompt?} We wondered whether high frequency words might be easier for the model to generate images from, and consequently that the metrics may be impacted by word frequency. We define the frequency of a prompt as the log of the average frequency of the words within the prompt. We use the SUBTLEX-US corpus to get frequency \citep{brysbaert2012adding} ratings for each word. We omit stopwords and assign the lowest frequency found in the corpus to any missing words. %Results are shown in Table \ref{tab:linguistic-corr-coco} and \ref{tab:ling-corr-winoground} for COCO and Winoground respectively.
% We find no correlation between prompt frequency for COCO or Winoground; specific numbers are omitted for space.



\newcommand{\tableCellLing}[1]{\rotatebox{80}{\parbox{4em}{ #1}}}
\newcommand{\tableCellVisual}[1]{\rotatebox{80}{\parbox{4em}{ #1}}}

\begin{table*}[!ht]
    \centering
    %{\small Spearman's Rank Correlation $\rho$ between Metrics and Linguistic Properties for COCO}\\[1.5ex]
    \begin{subtable}{\textwidth}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|llll |llll| llll}
    & \multicolumn{4}{c}{\parbox{15em}{$\rho$ -- Readability (Grade Level)\vspace*{1em}}}
    & \multicolumn{4}{c}{\parbox{15em}{$\rho$ -- Syntactic Complexity\vspace*{1em}}}
    & \multicolumn{4}{c}{\parbox{15em}{$\rho$ -- Length (\# of Words)}\vspace*{1em}} \\


    & \tableCellLing{CLIPScore}
    & \tableCellLing{TIFA}
    & \tableCellLing{VPEval}
    & \tableCellLing{DSG}
    
    & \tableCellLing{CLIPScore}
    & \tableCellLing{TIFA}
    & \tableCellLing{VPEval}
    & \tableCellLing{DSG}
    
    & \tableCellLing{CLIPScore}
    & \tableCellLing{TIFA}
    & \tableCellLing{VPEval}
    & \tableCellLing{DSG}
    \\\midrule
    
    %\hline
    Real Images & 0.28* & -0.30* & \bf -0.54* & \bf -0.44* & 0.23* & -0.36* & \bf -0.46* & \bf -0.44* & 0.29 & \bf -0.45* & \bf -0.76* & \bf -0.74*  \\
    
    \glide & -0.04 & -0.31* & \bf -0.63* & \bf -0.44* & -0.01 & -0.37* & \bf -0.41* & \bf -0.41* & -0.10 & \bf -0.66* & \bf -0.72* & \bf -0.77*  \\
    
    %glide\_bow & 0.19 & -0.38* & -0.45* & -0.38* & 0.08 & -0.30* & -0.37* & -0.29* & 0.39* & -0.59* & -0.69* & -0.76* & -0.93* & -0.93* & -0.93* & ~ \\
    
    \dalleshort & 0.33* & -0.22 & \bf -0.66* & \bf -0.40* & 0.15* & -0.39* & \bf -0.45* & \bf -0.48* & 0.28 & \bf -0.70* & \bf -0.80* & \bf -0.94*  \\
    
    \stablehf & \bf 0.49* & \bf -0.42* & \bf -0.56* & -0.30* & 0.10 & -0.34* & \bf -0.51* & \bf -0.48* & \bf 0.50* & \bf -0.74* & \bf -0.86* & \bf -0.91*  \\

    \stableapi & \bf 0.41* & -0.35* & -0.38* & -0.38* & 0.04 & -0.36* & \bf -0.50* & \bf -0.46* & \bf 0.42* & \bf -0.66* & \bf -0.69* & \bf -0.84*  \\\bottomrule
    
    \end{tabular}
    }
    \caption{Spearman's rank correlation between linguistic properties -- readability, complexity and length of text prompt -- and \metrics for COCO. Statistically significant values are marked with $*$. Moderate to strong statistically significant correlations are \textbf{in bold}. %See Table \ref{tab:ling-corr-winoground} for Winoground results.
    \Metrics are highly sensitive to linguistic features of the text.}
    \label{tab:linguistic-corr-coco}
    \end{subtable}
    
    \centering
    %{\small Spearman's Rank Correlation $\rho$ between Metrics and Visual Properties for COCO} \\
    
    
    \begin{subtable}{\textwidth}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l| llll| llll| llll}
    
    \multicolumn{1}{c}{}
    & \multicolumn{4}{c}{$\rho$ -- Concreteness}
    & \multicolumn{4}{c}{$\rho$ -- Imageability}
    & \multicolumn{4}{c}{\parbox{8em}{$\rho$ -- ImageNet-21k\\Caption Overlap}}\\

    & \tableCellVisual{CLIPScore}
    & \tableCellVisual{TIFA}
    & \tableCellVisual{VPEval}
    & \tableCellVisual{DSG}
    
    & \tableCellVisual{CLIPScore}
    & \tableCellVisual{TIFA}
    & \tableCellVisual{VPEval}
    & \tableCellVisual{DSG}
    
    & \tableCellVisual{CLIPScore}
    & \tableCellVisual{TIFA}
    & \tableCellVisual{VPEval}
    & \tableCellVisual{DSG}\\
    \toprule
    
    Real Images & 0.04* & -0.03 & 0.10* & -0.02 & -0.06* & 0.00 & 0.08* & 0.00 & -0.05 & -0.03 & 0.23 & 0.0 \\
    
    \glide & 0.03* & -0.05* & 0.00 & -0.04* & 0.12* & 0.05* & 0.10* & 0.06* & -0.12 & -0.08 & -0.05 & -0.07 \\ 
    
    % glide\_bow & 0.05* & -0.05* & -0.00 & -0.04* & 0.10* & 0.03* & 0.08* & 0.02 & 0.07 & -0.05 & 0.07 & -0.04 \\
    
    \dalleshort & 0.08* & -0.02 & 0.09* & -0.01 & -0.01 & 0.02 & 0.09* & 0.03* & 0.06 & -0.06 &  0.24 & 0.08 \\

    \stablehf & 0.02 & -0.03* & 0.09* & -0.03* & 0.02 & 0.02 & 0.10* & 0.02 & -0.04 & -0.04 & 0.23 & 0.11 \\
    
    \stableapi & 0.02 & -0.04* & 0.06* & -0.05* & 0.04* & 0.01 & 0.09* & 0.01 & 0.04 & -0.17 & -0.01 & 0.02 \\
    
    \bottomrule
    \end{tabular}
    }
    \caption{Spearman's rank correlation between visual properties and \metrics. Statistically significant values are marked with $*$. \Metrics are \textit{not} sensitive to the visual properties we evaluated.
    }
    \label{tab:visual-corr-coco}
    \end{subtable}
    
    \caption{Correlation for COCO between the \metrics and various standard linguistic properties are generally moderate to strong across models, while the correlation between the \metrics and various standard visual properties are predominantly weak. These results suggest \metrics are more language-related than vision related.% We do not find as strong correlations for visual features; see Table \ref{tab:visual-corr-coco} in the Appendix. 
    % We also observe similar patterns for the Winoground dataset; results are shown in Table \ref{tab:ling-corr-winoground} in the Appendix.
    %\textbf{Takeaway:} \Metrics are sensitive to linguistic properties of the text prompt, showing moderate to strong correlation. However, these properties do not appear to be sensitive to visual properties.
    }
\end{table*}




\section{Experiment 2: Relationship with visual properties}\label{sec:corr-visual}

We also ran analyses of visually important features, as proxied by the text prompt. The visual features include the \textbf{imageability}, \textbf{concreteness} and \textbf{overlap with ImageNet-21k (IN-21k) object classes} \citep{ridnik2021imagenet}. We use the concreteness ratings for 40k words provided by \citet{brysbaert2014concreteness} to approximate a concreteness score for each prompt. We use the lowest concreteness score in the corpus for any missing words. Imageability describes how easily hearing a word leads to creating a mental image \citep{paivio1968concreteness,bird2001age}. We use imageability scores from \citet{gao2023scope} and assign missing words the lowest score in the corpus. \footnote{For concreteness and imageability scoring, we also ran an experiment where we assigned missing words a score of 0 and where we omitted missing words. We did not observe a signficant difference in the correlations.} Lastly, for IN-21k, we compute the percent overlap between the words in the caption and the objectsclasses, excluding stopwords. %Given the use of IN21k by many vision models, hypothesize that text prompts that include IN21k should be easier for T2I models to generate and should therefore have higher \metrics scores.

See Table \ref{tab:visual-corr-coco} for COCO results and \ref{tab:visual-corr-winoground} in the Appendix for Winoground results. Because language provides such a strong prior in vision-language tasks like VQA \citep{zhang2016yin,goyal2017making,agrawal2018CVPR, lin2024revisiting}, we wanted to ensure the visual modality was being used in these metrics. We found that there is essentially no correlation between the \metrics and the visual properties we evaluated. % Because all investigated evaluation metrics have medium to high significant correlations with linguistic features, we focus our energy in the rest of the paper on the language side, as that seems to be more likely to influence evaluation metrics' performance.



\paragraph{Do evaluation metrics correlate with prompt concretetess?}\label{sec:concreteness} 
Are prompts that describe more concrete words and concepts more accurately generated? We use the concreteness ratings for 40k words provided by \citet{brysbaert2014concreteness} to approximate a concreteness score for each prompt. We use the lowest concreteness score in the corpus for any missing words.

\paragraph{Do evaluation metrics correlation with prompt imageability?}
Imageability describes how easily hearing a word leads to creating a mental image \citep{paivio1968concreteness,bird2001age}. We use imageability scores from \citet{gao2023scope}. We follow the same approach as we did in Section \ref{sec:concreteness} to handle prompts that contain words without an associated imageability score. While we expected that more imageable prompts would correlate with higher \metrics scores, we did not observe this.

\paragraph{Do evaluation metrics correlate with the number of objects in an image?}

ImageNet21k (IN21k; \citealt{deng2009imagenet}) is a dataset of 14M images and 21k different labels. This dataset has been used for pretraining and finetuning many vision models (\eg \citealt{steiner2021train,zhou2022detecting}). For this reason, we explore whether captions that have a high overlap with classes in IN21k correlate with higher performance. We hypothesize that text prompts that include IN21k should be easier for T2I models to generate and should therefore have higher \metrics scores.



\section{Experiment 3: How distinct are these metrics?}\label{sec:metrics-distinct}

% First, new metrics should not correlate super highly with old metrics (unless they are significantly cheaper to run, easier to interpret, etc.). We investigate this question and find \TODO{}. We also explore what information is being conveyed by these metrics and evaluate the extent to which these new T2I consistency metrics actually convey new information, or just reflect factors of their input prompts.
%\subsection{Contribution of each new metric}

%\subsection{Relationship between each metric}
First, when a new evaluation metric is proposed, we should first check to be sure that it improves upon the state of the art, in other words, it should probe new information (or be able to probe old information in a better way). We investigate the extent to which new VQA-based metrics convey similar information to existing metrics (CLIPScore) and each other, quantifying similarity as Spearman's rank correlation. For generate images for every prompt in %$\mathcal{D}_{COCO}$ and $\mathcal{D}_{Winoground}$ 
COCO and Winoground across the 5 different T2I models and using the real images. Then, we compute the scores for metrics (CLIPScore, TIFA, VPEval and DSG) and then measure the pairwise Spearman's correlation between the metrics. Results are shown in Figure \ref{fig:exp3-coco}.

% \TODO{AW: explain correlation as contributing more than CLIP (not less)}

\textbf{We find strong, statistically significant correlation between each of the VQA-based metrics.} This may be due to either 1) similar approaches to generating questions using an external LM or 2) similar approaches to evaluation by using a VQA model. CLIPScore shows the weakest correlation, which is likely because it operates using cosine similarity instead. This leads us to question -- how can we ensure new VQA-based evaluation metrics introduce or leverage new information?



\begin{figure*}[hb!]
    \centering
    \hspace*{-1em}
    \begin{tikzpicture}
    % top row
    \node(real-images){
        \includegraphics[width=10em]{coco_heatmap_real_filtered.png}
    };
    \node[right=-3em of real-images](dalle2){
        \includegraphics[width=10em]{coco_heatmap_dalle2.png}
    };
    \node[right=-3em of dalle2](glide){
        \includegraphics[width=10em]{coco_heatmap_glide.png}
    };
    \node[right=-3em of glide](sd-hf){
        \includegraphics[width=10em]{coco_heatmap_sd_hf.png}
    };
    \node[right=-3em of sd-hf](sd-api){
        \includegraphics[width=10em]{coco_heatmap_sd_api.png}
    };
    \end{tikzpicture}
    
    \caption{Correlation between each pair of \metrics for COCO. The VQA-based metrics are not highly correlated with CLIPScore (with the exception of GLIDE), and that correlations with real images resemble those from generated images. For VQA-based metrics, correlations are medium to strong and statistically significant, suggesting these metrics may be interchangeable. We observe weaker yet broadly similar trends for Winoground; results are shown in Figure \ref{fig:exp3-winoground}. % \textbf{Takeaway: The VQA-based \metrics have moderate and strong correlations for real and generated images.}
    }
    \label{fig:exp3-coco}
\end{figure*}

